Building Concise Logical Patterns by Constraining Tsetlin Machine Clause Size

Tsetlin machine (TM) is a logic-based machine learning approach with the crucial advantages of being transparent and hardware-friendly. While TMs match or surpass deep learning accuracy for an increasing number of applications, large clause pools tend to produce clauses with many literals (long clauses). As such, they become less interpretable. Further, longer clauses increase the switching activity of the clause logic in hardware, consuming more power. This paper introduces a novel variant of TM learning - Clause Size Constrained TMs (CSC-TMs) - where one can set a soft constraint on the clause size. As soon as a clause includes more literals than the constraint allows, it starts expelling literals. Accordingly, oversized clauses only appear transiently. To evaluate CSC-TM, we conduct classification, clustering, and regression experiments on tabular data, natural language text, images, and board games. Our results show that CSC-TM maintains accuracy with up to 80 times fewer literals. Indeed, the accuracy increases with shorter clauses for TREC, IMDb, and BBC Sports. After the accuracy peaks, it drops gracefully as the clause size approaches a single literal. We finally analyze CSC-TM power consumption and derive new convergence properties.

==> architecture.tex <==
\section{Parallel and Asynchronous Architecture}\label{sec:architecture}
Even though CPUs have been traditionally geared to handle high workloads, they are more suited for sequential processing and their performance is still dependant on the limited number of cores available. In contrast, since GPUs are primarily designed for graphical applications by employing many small processing elements, they offer a large degree of parallelism \cite{owens2007survey}. As a result, a growing body of research has been focused on performing general purpose GPU computation or GPGPU. For efficient use of GPU power, it is critical for the algorithm to expose a large amount of fine-grained parallelism \cite{jiang2005automatic,satish2009designing}.

The inherent discreetness of the \ac{TM} architecture allows us to effectively use the parallel processing power of GPUs to offer a huge speedup over the existing implementations. In this section, we introduce our decentralized inference scheme and the accompanying architecture that makes it possible to have parallel asynchronous learning and classification.

\subsection{Voting Tally}

A voting tally that tracks the aggregated output of the clauses for each training example is central to our scheme. In a standard \ac{TM}, each training example $(X_i, y_i), 1 \le i \le N,$ is processed by first evaluating the clauses on $X_i$ and then obtaining the majority vote $v$ from Eq.~(\ref{eqn:aggregated_votes}). Here $N$ is the total number of examples. The majority vote $v$ is then compared with the summation target $T$ when $y=1$ and $-T$ when $y=0$, to produce the feedback to the \acp{TA} of each clause.

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/MassiveParallel.png}
\caption{Parallel Tsetlin machine architecture.}\label{figure:architecture_basic}
\end{figure}

As illustrated in Fig.~\ref{figure:architecture_basic}, to decouple the clauses, we now assume that the particular majority vote of example $X_i$ has been pre-calculated, meaning that each training example becomes a triple $(X_i, y_i, v_i)$, where $v_i$ is the pre-calculated majority vote. With $v_i$ in place, the calculation performed in Eq.~(\ref{eqn:aggregated_votes}) can be skipped, and we can go directly to give Type I or Type II feedback to any clause $C_j$, without considering the other clauses. This opens up for decentralized learning of the clauses. 
However, any time the composition of a clause changes after receiving feedback, all voting aggregates $v_i, 1 \le i \le N,$ becomes outdated. This requires that the standard learning scheme for updating the clauses must be replaced.

\begin{algorithm}[t]
%\scriptsize
\small
\caption{Decentralized updating of clause}
\label{alg:decentralized_clause_updating}

\Input{Example pool $P$, clause $C_j$, positive polarity indicator $p_j \in \{\False, \True\}$, batch size $b \in [1,\infty)$, voting target $T \in [1,\infty)$, pattern specificity $s \in [1.0, \infty)$}

\begin{algorithmic} [1]
\Procedure{UpdateClause}{$C_j, p_j, P, b, T, s$}

\For{$i \gets 1, \ldots, b$}
    \State $(X_i, y_i, v_i) \gets \mathrm{ObtainTrainingExample}(P)$
    \State $v_i^c \leftarrow \mathbf{clip}\left(v_i, -T, T\right)$
    \State $e = T - v_i^c \mathbf{~if~} y_i = 1 \mathbf{~else~} T + v_i^c$ 

    \If{rand() $\le \frac{e}{2T}$}
        \If{$y_i \mathbf{~xor~} p_j$}
            \State TypeIIFeedback($X_i, C_j$)
        \Else
            \State TypeIFeedback($X_i,  C_j, s$)
        \EndIf 
    
        \State $o_{ij} \gets C_j(X_i)$
        \State $o_{ij}^{*} \gets \mathrm{ObtainPreviousClauseOutput}(i,j)$
        \If{$o_{ij} \ne o_{ij}^{*}$}
            \State $\mathrm{AtomicAdd}(v_i, o_{ij} - o_{ij}^{*})$
            \State $\mathrm{StorePreviousClauseOutput}(i,j, o_{ij})$
        \EndIf
    \EndIf
\EndFor

\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Decentralized Clause Learning}

Our decentralized learning scheme is captured by Algorithm~\ref{alg:decentralized_clause_updating}. As shown, each clause is trained independently of the other clauses. That is, each clause proceeds with training without taking other clauses into consideration. Accordingly, Algorithm~\ref{alg:decentralized_clause_updating} supports massive parallelization because each clause can now run in its own thread.

Notice further how the clause in focus first obtains a reference to the next training example $(X_i, y_i, v_i)$ to process, including the pre-recorded voting sum $v_i$ (Line 3). This example is retrieved from an example pool $P$, which is the storage of the training examples (centralized or decentralized).

The error of the pre-recorded voting sum $v_i$ is then calculated based on the voting target $T$ (Line 5). The error, in turn, decides the probability of updating the clause. The  updating rule is the standard Type I and Type II \ac{TM} feedback, governed by the polarity $p_j$ of the clause and the specificity hyper-parameter $s$ (Lines 6-11).

The moment clause $C_j$ is updated, all recorded voting sums in the example pool $P$ are potentially outdated. This is because $C_j$ now captures a different pattern. Thus, to keep all of the voting sums $v_i$ in $P$ consistent with $C_j$, $C_j$ should ideally have been re-evaluated on all of the examples in $P$.

To partially remedy for outdated voting aggregates, the clause only updates the \emph{current} voting sum $v_i$. This happens when the calculated clause output $o_{ij}$ is different from the previously calculated clause output $o_{ij}^*$ (Lines 12-17). Note that the previously recorded output $o_{ij}^*$ is a single bit that is stored locally together with the clause. In this manner, the algorithm provides \emph{eventual consistency}. That is, if the clauses stop changing, all the voting sums eventually become correct.

Employing the above algorithm, the clauses access the training examples simultaneously, updating themselves and the local voting tallies in parallel. There is no synchronization among the clause threads, apart from atomic adds to the local voting tallies (Line 15). Accordingly, with this minimalistic synchronization, each team of \acp{TA} will usually operate on partially calculated or outdated voting tallies.

==> empirical_results_rupsa.tex <==
\subsection{Rupsa}
What happens when we reduce the clause size b?
Accuracy/Interpretability

no.of clauses == best as with no budgeting 

budget vs accuracy

budget vs learning time

with/without budget  vs average no. of literals per clause


NLP :: showing example clauses
--YELP
--Hate


Find your max clause length using Vanilla TM. Go down by half every round till you reach >=1 .

Vision
--MNIST
--FashionMNIST

Better reconstruction with smaller clauses??


Size of final model in kBs.




==> hardware_and_energy_considerations.tex <==
\section{Hardware Complexity and Energy Consumption Analysis}

TM hardware accelerators will typically be implemented by either Field Programmable Gate Arrays~(FPGAs) or Application Specific Integrated Circuits~(ASICs). In most cases the dominating part of the energy consumption is related to the switching of digital circuits. It should be noted, however, that the static power consumption due to transistor leakage current for high performance processes can reach up to 30\% of total power~\cite{Dally}. With implementations in low power processes the static power consumption will be much less.

The dynamic power, $P$, consumed by a digital circuit with load capacitance $C$, operating frequency $f$, supply voltage $V_{S}$, and an activity factor $\alpha$ (transitions per clock cycle) is given by Eq.~(\ref{equation: swithcing power consumption})~\cite{Dally},
\begin{equation} \label{equation: swithcing power consumption}
\textstyle
P=0.5 \times C \times V_{S}^2 \times f \times \alpha.
\end{equation}\noindent
Limiting the number of literals will reduce the $\alpha$ value in several gates that implement the clause logic. Only those gates that process the included literals will switch and consume energy. The reduction in energy consumption of the clause logic can therefore roughly be estimated to $\frac{\bf{b}}{l_{ave}}$, where $\bf{b}$ is the clause size constraint and $l_{ave}$ is the average number of literals in the model without the length constraint. The exact savings will depend on the dataset.


% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.7\linewidth]{figures/Clause_logic.pdf}
% \caption{Hardware implementation of clause logic based on a) the classical approach and b) multiplexers.}\label{figure:Clause_logic}
% \end{figure}

% Figure \ref{figure:Clause_logic_classical} shows two alternative solutions for hardware implementation of a clause. Both can be used for literal budgeting. In this example there are 272 literals, and the number of literals per clause is limited to four.

The classical approach~\cite{wheeldon2020learning} for implementing clause logic is shown in Figure~\ref{figure:Clause_logic_classical}. 
Here each literal ${l_1, \ldots,l_{2o}}$ is either included or excluded by the associated include signal ${i_1, \ldots,i_{2o}}$ (active low) by using OR-gates. The include signals will typically all be simultaneously available from a register. The outputs from the OR-gates are then fed to a wide-input AND-gate, which will normally be implemented by several smaller AND-gates connected in a tree-structure to reduce path delay. Clearly, for a certain fixed application, given a smaller number of included literals, we can reduce the number of OR-gates to $\bf{b}$, and use an AND gate with only $\bf{b}$ inputs. In this way, the hardware complexity and power consumption can be reduced. 
For a general case, where the TM needs to be programmable in distinct applications, we need to have sufficient amount of available literals. Nevertheless, CSC-TM still has benefits in reduced switching activity, thus saving power.


\begin{figure}[ht]
\centering
\includegraphics[width=0.5\linewidth]{figures/Clause_logic_classical.pdf}
\caption{Hardware implementation of clause logic.}\label{figure:Clause_logic_classical}
\end{figure}

% Figure \ref{figure:Clause_logic} b) shows an alternative solution based on multiplexers. Here four 272-to-1 multiplexers feed the included literals to the AND-gate. Four address signals select which literals are included. In the special case that no literals are included, the \textit{Empty\_n} signal (active low) forces the clause output $c_j$ to 0. What is also needed (but not shown on Figure \ref{figure:Clause_logic} b)) is a special address to the multiplexers that feeds a logical 1 to the AND-gate in the case a literal is not included. This is required, for instance, if only a three out of four literal are included in the clause. 

% Which solution will require the least amount of hardware resources depends on the amount of literals and the maximum number of literals, $\bf{b}$, used during literal budgeting. With a huge number of literals, $l$, and small $\bf{b}$, the multiplexer-based solution can be more suitable. However, in many cases the classical approach will be preferred even if the AND-functions needs to be very wide. This is because the logic needed for the multiplexers is significant when many literals are available. 

% For very high operating frequency one will sometimes need to use pipelining of circuit functions to avoid long signal path delays. This comes at the expense of latency. The multiplexer-based solution can more easily be designed without pipelining compared to the classical approach.

% With a fixed/frozen model there can be significant savings in hardware resources and energy consumption as the included literals can be directly connected to the AND gate, and many logical gates can be omitted from the design.

% TBD: Mention that even without literal budgeting, if the model includes only a few include bits for each clause, the switching noise will be significantly reduced compared to a situation where many literals are included. However, in this case there is no hardware resource savings, and the leakage current from all the logic is not reduced.

It should be noted that it is only the energy consumption related to the clause logic that is affected by constraining clause size. The ensuing hardware processing, e.g., with clause weighting and summation is not affected. However, for systems with a huge number of clauses, the clause logic will occupy a significant part of the digital circuitry, and reducing its switching activity can enable significant energy savings.

An important system level benefit of literal budgeting is the time required for a model to be loaded from external or on-chip memory into registers in the ASIC or FPGA.  During this time the system's processor and the data transfer itself will consume energy. With less included literals, the model size and thus the load time can be reduced with a suitable encoding scheme, such as Run Length Encoding (RLE)~\cite{BakarRahman}. Reduction of the model size is also beneficial for other embedded TM solutions based on low-power microcontrollers.

% Finally, for submicron integracted circuit (IC) technologies, the static power consumption caused by leakage current can be significant. To reduce this one can use transistors with higher threshold voltages, at the expense of lower speed or higher supply voltage. To reduce the static energy consumption of the clause logic, one should use the solution that results in the smallest number of logical gates. 
